Are Normalizing Flows the Key to Unlocking the Exponential Mechanism?

The Exponential Mechanism (ExpM), designed for private optimization, has been historically sidelined from use on continuous sample spaces, as it requires sampling from a generally intractable density, and, to a lesser extent, bounding the sensitivity of the objective function. Any differential privacy (DP) mechanism can be instantiated as ExpM, and ExpM poses an elegant solution for private machine learning (ML) that bypasses inherent inefficiencies of DPSGD. This paper seeks to operationalize ExpM for private optimization and ML by using an auxiliary Normalizing Flow (NF), an expressive deep network for density learning, to approximately sample from ExpM density. The method, ExpM+NF is an alternative to SGD methods for model training. We prove a sensitivity bound for the $\ell^2$ loss permitting ExpM use with any sampling method. To test feasibility, we present results on MIMIC-III health data comparing (non-private) SGD, DPSGD, and ExpM+NF training methods' accuracy and training time. We find that a model sampled from ExpM+NF is nearly as accurate as non-private SGD, more accurate than DPSGD, and ExpM+NF trains faster than Opacus' DPSGD implementation. Unable to provide a privacy proof for the NF approximation, we present empirical results to investigate privacy including the LiRA membership inference attack of Carlini et al. and the recent privacy auditing lower bound method of Steinke et al. Our findings suggest ExpM+NF provides more privacy than non-private SGD, but not as much as DPSGD, although many attacks are impotent against any model. Ancillary benefits of this work include pushing the SOTA of privacy and accuracy on MIMIC-III healthcare data, exhibiting the use of ExpM+NF for Bayesian inference, showing the limitations of empirical privacy auditing in practice, and providing several privacy theorems applicable to distribution learning.

==> 85-related-works.tex <==
\section{Related Works}
Background work for DP, DPSGD, and NFs is discussed in the Introduction \ref{sec:intro}, Background sections \ref{sec:background} and their related Appendices. 
Here we itemize other works and their relationship to this paper. 

A concurrent work by Lin et al. \cite{lin2024tractable} as well as previous works, e.g., \cite{gopi2022private}, provide mathematical treatment of using MCMC methods to sample from  ExpM for model training.
Yet, these works provide no implementation of the proposed method, and hence no empirical testing of computational efficiency or accuracy, e.g., against DPSGD. 
The main benefit / limitation of our work---computationally promising results / inability to prove privacy---is seemingly flipped with these works, as their benefit is  proof of privacy but, they offer no implementation nor any testing against the state of the art.  

Examples of using  ExpM for differentially private ML in the finite setting exist,  e.g.:  \cite{friedman2010data} (private decision tree with only categorical features), \cite{kapralov2013differentially} (private PCA), and \cite{vinterbo2012differentially} (private feature selection with only categorical variables). 
Notwithstanding these examples, ExpM is historically intractable in most ML applications as the optimization is of a loss function over  continuous parameter space \cite{kasiviswanathan2011what, ji2014differential, minami2016differential,  near2022programming}.

Works to investigate   NF expressiveness exist \cite{kong2020expressive, lu2020universal, verine2023on}. 
These provide existence  theorems guaranteeing an NF of a particular form can / cannot approximate a target density of a particular form. 
They are tangential to this work as  ExpM+NF privacy  requires  proof that the trained NF's output density is, for any training dataset, a good approximation of the target. 


